A Secretary Problem with a Sliding Window for Recalling Applicants

The Sliding Window Secretary Problem allows a window of choices to the Classical Secretary Problem, in which there is the option to choose the previous $K$ choices immediately prior to the current choice. We consider a case of this sequential choice problem in which the interviewer has a finite, known number of choices and can only discern the relative ranks of choices, and in which every permutation of ranks is equally likely. We examine three cases of the problem: (i) the interviewer has one choice to choose the best applicant; (ii) the interviewer has one choice to choose one of the top two applicants; and (iii) the interviewer has two choices to choose the best applicant. The form of the optimal strategy is shown, the probability of winning as a function of the window size is derived, and the limiting behavior is discussed for all three cases.

==> summary.tex <==
We examine a famous problem in mathematics, the Secretary Problem, in which an interviewer tries to select the best applicant in a sequence of applicants for a job, but can only interview each applicant once and has to accept or reject each applicant immediately after the interview. We generalize this problem to a Sliding-Window Secretary Problem in which the interviewer can choose from a window of the previous applicants, so that the problem can more realistically model data stream mining.  We study two cases of the Sliding-Window Secretary Problem and fully characterize their solutions along with important trends in the solutions.
